Voliro: An Omnidirectional Hexacopter With Tiltable Rotors

Extending the maneuverability of unmanned areal vehicles promises to yield a considerable increase in the areas in which these systems can be used. Some such applications are the performance of more complicated inspection tasks and the generation of complex uninterrupted movements of an attached camera. In this paper we address this challenge by presenting Voliro, a novel aerial platform that combines the advantages of existing multi-rotor systems with the agility of omnidirectionally controllable platforms. We propose the use of a hexacopter with tiltable rotors allowing the system to decouple the control of position and orientation. The contributions of this work involve the mechanical design as well as a controller with the corresponding allocation scheme. This work also discusses the design challenges involved when turning the concept of a hexacopter with tiltable rotors into an actual prototype. The agility of the system is demonstrated and evaluated in real- world experiments.

==> Makefile <==
# The target that we want to build, TODO: change name if required
targets=main.pdf

# Dependencies, all files which are taken into consideration when make decides
# if rebuilding is necessary
deps=$(wildcard */*.tex) $(wildcard figures/*.png) $(wildcard figures/*.jpg) \
	$(wildcard figures/*.jpeg) $(wildcard figures/*.pdf) \
	$(wildcard *.bib)

# NOTE: you should not change anything below
%.pdf: %.tex $(deps) Makefile build
	# cd to build and build the report
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex $<
	cd build && BIBINPUTS=../:${BIBINPUTS} BSTINPUTS=../:${BSTINPUTS} bibtex $*
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex $<
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex $<
	# copy the resulting pdf back to the main directory (mv is no good, because
	# make will rebuild even if nothing has changed)
	cp build/$@ .

all: $(targets)

clean: buildclean

build:
	# make sure that build exists
	mkdir -p build

buildclean:
	# remove the build folder
	rm -rf build *~ */*~

distclean: clean
	# remove the build folder (clean) and the target pdf
	rm -f $(targets)

installdeb:
	# required packages to use this makefile
	sudo apt-get install texlive texlive-math-extra texlive-publishers

.PHONY: clean buildclean distclean all dist installdeb

